Ares II: Tracing the Flaws of a (Storage) God

Ares is a modular framework, designed to implement dynamic, reconfigurable, fault-tolerant, read/write and strongly consistent distributed shared memory objects. Recent enhancements of the framework have realized the efficient implementation of large objects, by introducing versioning and data striping techniques. In this work, we identify performance bottlenecks of the Ares's variants by utilizing distributed tracing, a popular technique for monitoring and profiling distributed systems. We then propose optimizations across all versions of Ares, aiming in overcoming the identified flaws, while preserving correctness. We refer to the optimized version of Ares as Ares II, which now features a piggyback mechanism, a garbage collection mechanism, and a batching reconfiguration technique for improving the performance and storage efficiency of the original Ares. We rigorously prove the correctness of Ares II, and we demonstrate the performance improvements by an experimental comparison (via distributed tracing) of the Ares II variants with their original counterparts.

==> pseudocode-clientjoin.tex <==
\myparagraph{\large{Configuration Initialization}.}
A service can act as a central point of control for managing the initial configuration. It should maintain a list of active servers in the system.
When new clients join the system can contact this service to obtain the current initial configuration, which they can use as their starting point.
However, we must ensure that the service itself is scalable and resilient to avoid becoming a single point of failure. 
Consensus is a good choice because even if some nodes fail, it keeps the configuration intact and available and ensures that the clients have an accurate starting point.
Also, since not many clients want to change the configuration simultaneously, we can handle the resource-intensive nature of this service without much hassle.
We already have an external Raft consensus-based (leader-follower) service for reconfiguration as defined in Section~\ref{ssec:optimization:reconfig}. As we mentioned this service operates as a $Key-Value$ storage, with keys representing config IDs and values corresponding to configurations. 
We can leverage this RAFT service to also inform clients about the last configuration.
We consider this RAFT service initialized with a configuration of servers. When a client executes an operation for the first time, they must first join the system. Thus, the client issues a query to the RAFT service to retrieve the latest configuration (line  Alg.~\ref{algo:read_writeProtocol}:~\ref{line:client-join:get-max}). 
The RAFT service should respond with the latest finalized configuration and its id, identified by the maximum key with a status of $F$, where the key represents the configuration ID.  A finilized configuration is essential to ensure that all data are included. However, this RAFT service is not updated with the value of the status, as the decision is made before the transfer of the data. So during the \act{finalize-config} action, we have to inform the RAFT servers of the $F$ status of the configuration executing $Con.{\act{finalize-config}}(\lambda)$ before the action completes. 
% (lines Alg.~\ref{algo:reconfigurer}:\ref{line:finalize:RAFT}).
% (e.g., the id is equal to j, where $cseq[j]$ represents a configuration at the client).
Then the client initializes its configuration sequence ($cseq$) with the most recent configuration, using its id as the index in the list, ensures that the client starts with the latest agreed-upon configuration (Alg.~\ref{algo:read_writeProtocol}:~\ref{line:client-join:initCseq}). 


==> pseudocode-join_depart.tex <==
\cgnote{I think we should remove this section.}

In this section, to enhance liveness of the service we introduce two new operations: \act{join} and \act{depart}. When a new device $c$ wishes to become a server in the system, it initiates a $\act{server-join}(c)$ action.
% in the USER layer. 
Conversely, when an old device intends to leave, it initiates a $\act{server-depart}(c)$. 
First, the $\act{server-join}$ performs a 
% $\act{get-last-config}$ 
$\act{get-max}$ on the RAFT service (cf. Section~\ref{appendix:optimizations:initCseq})
to obtain the most recent finalized configuration (line Alg.\ref{algo:server-join+depart}:\ref{line:join:get-max}).
% (line Alg.\ref{algo:server-join+depart}:\ref{line:join:get-last-config}). 
% The $\act{get-last-config}$ is defined in DSMM layer (line Alg.~\ref{algo:read_writeProtocol}:\ref{line:join:get-last-config}). It simply executes a $\act{read-config}$ request to update its $cseq$ and returns the latest finalized entry to USER layer. 
Once the $\act{server-join}$ operation becomes aware of the last finalized configuration $c_{cur}$, it initiates an HTTP request to an external monitoring service to acquire updates on the health status of servers within $c_{cur}$ (line Alg.\ref{algo:server-join+depart}:\ref{line:join:monitor}). The monitoring service evaluates each server in $c_{cur}$ and verifies its connectivity. Subsequently, it generates a $statuses$ list that includes the servers, each marked with a number, either $0$ or $1$, to indicate the server's health.
Finally, the $\act{server-join}$ operation executes a $\act{reconfig}$ operation to propose a new configuration that includes only the healthy servers, as determined by the monitor, and the device seeking to join (line Alg.\ref{algo:server-join+depart}:\ref{line:join:recongig}). If the $\act{reconfig}$ operation does not succeed, it indicates that the configuration agreed upon by consensus is different from the proposed configuration that includes server $c$. The above procedure is repeated until the server $c$ successfully joins the system. The $\act{server-depart}(c)$ is identical to the $\act{server-join}(c)$ operation, with the only difference that it removes the server from the proposed interval instead of adding it.

\begin{algorithm}[!htbp]
            \footnotesize
			\begin{multicols}{2}
			\begin{algorithmic}[1]\footnotesize
				\State {\bf State Variables:}
                \Statex $statuses \subseteq \srvSet{} \times \{0,1\}$, initially $\{\}$
				
    %             \Statex

    %             \JDboxParam{0.7}{
    %             \Procedure{update-cseq}{} 
				% \State $id,c\gets Con.\text{get-max()}$ \label{line:update-cseq:get-max}
				% \State $cseq[id]\gets c$
    %             \label{line:update-cseq:updateCseq}
    %             \State $\mu\gets id$
    %             \State {\bf return} $cseq[id]$
    %             \EndProcedure
                
    %             \Statex

    %             \Procedure{get-last-config}{$cseq$} 
    %             \State $cseq,\mu,\_ \gets$\act{read-config}($cseq,\mu,True$)
    %             % \State $\mu\gets\max(\{i: cseq[i].status = F\})$
				% \State {\bf return} $\servers{cseq[\mu]}$
    %             \EndProcedure
    %             }

                \Statex

                % \JDboxParam{0.7}{
                \Operation{server-join}{c}\label{server-join}
                \State $status \gets False$
                \While{$status==False$}
                % \State $c_{cur} \gets \act{get-last-config}()$ \label{line:join:get-last-config}
                \State $id,c_{cur}\gets Con.\text{get-max()}$ \label{line:join:get-max}
                \State $statuses \gets \act{health-monitor}(c_{cur})$ \label{line:join:monitor}
                \State $c_{live} \gets [s: statuses[s] = 1]$ \label{line:join:healthservers}
                \State $status \gets \act{reconfig}(c_{live} \cup c)$ \label{line:join:recongig}
                \EndWhile
                
			\EndOperation
                % }

                \Statex
                
            % \JDboxParam{0.75}{
			\Operation{server-depart}{c}\label{server-depart}
                \State $status \gets False$
                \While{$status==False$}
                % \State $c_{cur} \gets \act{get-last-config}()$
                \State $id,c_{cur}\gets Con.\text{get-max()}$ \label{line:depart:get-max}
                \State $statuses \gets \act{health-monitor}(c_{cur})$
                \State $c_{live} \gets [s: statuses[s] = 1]$
                \State $status \gets \act{reconfig}(c_{live} \backslash~c)$  
                \EndWhile
			\EndOperation
                % }
\end{algorithmic}
	\end{multicols}
	\caption{Server's Join and Depart protocols.} 
 % at USER level.
    \label{algo:server-join+depart}
\end{algorithm}          




==> pseudocode_ConfigurationDiscovery.tex <==
% \input{pseudocode-clientjoin}
% Alternative Approach for update $cseq$
% Another drawback is that \ares{} starts with an initial configuration of servers, and new clients join this configuration. However, we are concerned about the possibility of server failures. 
% In this case, clients may not find a live configuration following the sequence of configurations.

% Then the client initializes its configuration sequence ($cseq$) with the most recent configuration, using its id as the index in the list, ensures that the client starts with the latest agreed-upon configuration (Alg.~\ref{algo:read_writeProtocol}:~\ref{line:client-join:initCseq}). 
\cgnote{Should we remove this section?}
In \ares{} new clients start their operations with a configuration sequence $cseq$ which is initialized with the configuration $c_0$. 
However the $c_0$ may become unresponsive. The same can happen in a following configuration, so the client cannot following the sequence of configurations.
So, when a client join the system for the first time, they need to obtain a live configuration, which they can use as their starting point.
Also, we have to implement timeouts for configuration requests to prevent indefinite waiting. When a client cannot receive a response within a specific time, it need to obtain a recent live configuration. 


A service can act as a central point of control for managing configurations and maintain a list of active servers in the system.
However, we must ensure that this service is scalable and resilient to avoid becoming a single point of failure. 
Consensus is a good choice because, even if some nodes fail, it keeps the configuration intact and available and ensures that the clients have an accurate starting point.
Also, since not many clients want to change the configuration simultaneously, we can handle the resource-intensive nature of this service without much hassle.
We already have an external Raft consensus-based (leader-follower) service for reconfiguration, as defined in Section~\ref{ssec:optimization:reconfig}. This service operates as a $Key-Value$ storage, with keys representing configuration IDs and values corresponding to configurations. 
We can leverage this RAFT service to also inform clients about the last configuration.
We consider this RAFT service initialized with the configuration of servers $c_0$. 
When a client wants to join the system or it does not receive a response within a specific time while is already a part of the system, it executes an \act{update-cseq} operation (line  Alg.~\ref{algo:client_init}:~\ref{line:update-cseq:get-max}).
This operation issues a query to the RAFT service to retrieve the latest configuration. 
The RAFT service should respond with the latest finalized configuration and its ID, identified by the maximum key with a status of $F$, where the key represents the configuration ID.  A finalized configuration is essential to ensuring that all data are included. However, this RAFT service is not updated with the value of the status, as the decision is made before the transfer of the data. So during the $\act{finalize-config}$ action, we have to inform the RAFT servers of the $F$ status of the configuration executing $Con.{\act{finalize-config}}(\lambda)$ before the action completes.  
% (line Alg.~\ref{algo:reconfigurer}:\ref{line:finalize:RAFT}).
% (e.g., the id is equal to j, where $cseq[j]$ represents a configuration at the client).
Then the client updates its configuration sequence ($cseq$) with the most recent configuration, using its id as the index in the list, ensuring that the client starts with the latest agreed-upon configuration (Alg.~\ref{algo:client_init}:\ref{line:update-cseq:updateCseq}). 

\begin{algorithm*}[!ht]
	%\hrule \F
	\begin{algorithmic}[2]
        \footnotesize
		\begin{multicols}{2}{\footnotesize
				\State at each writer $w_i$ and reader $r_i$

				\State {\bf State Variables:}
				\State  $cseq[]~s.t.~cseq[j]\in\confSet\times\{F,P\}$ 
				\State {\bf Initialization:} 
				\State $cseq[0] = \tup{c_0,F}$ 

                \Statex

                \Procedure{update-cseq}{} 
				\State $id,c\gets Con.\text{get-max()}$ \label{line:update-cseq:get-max}
				\State $cseq[id]\gets c$ \label{line:update-cseq:updateCseq}
                \State {\bf return} $cseq[id]$ 
                \EndProcedure
                % \Statex
    %             \Procedure{get-last-config}{$cseq$} 
    %             \State $cseq \gets$\act{read-config}($cseq$)
    %             \State $\mu\gets\max(\{i: cseq[i].status = F\})$
				% \State {\bf return} $\servers{cseq[\mu]}$
    %             \EndProcedure
    %             }   
    }\end{multicols}
   \end{algorithmic}
	\caption{Client Initialization in \ARESopt{}.}
	\label{algo:client_init}
\end{algorithm*}
